TriSum: Learning Summarization Ability from Large Language Models with Structured Rationale

The advent of large language models (LLMs) has significantly advanced natural language processing tasks like text summarization. However, their large size and computational demands, coupled with privacy concerns in data transmission, limit their use in resource-constrained and privacy-centric settings. To overcome this, we introduce TriSum, a framework for distilling LLMs' text summarization abilities into a compact, local model. Initially, LLMs extract a set of aspect-triple rationales and summaries, which are refined using a dual-scoring method for quality. Next, a smaller local model is trained with these tasks, employing a curriculum learning strategy that evolves from simple to complex tasks. Our method enhances local model performance on various benchmarks (CNN/DailyMail, XSum, and ClinicalTrial), outperforming baselines by 4.5%, 8.5%, and 7.4%, respectively. It also improves interpretability by providing insights into the summarization rationale.

==> tables/perf_llm_reference.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!h]
\small
\centering
% \setlength{\tabcolsep}{3.9pt}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
  \multicolumn{4}{c}{\textbf{CNN/DailyMail}}    \\      
\textbf{Model} & \textbf{R-1}   & \textbf{R-2}   & \textbf{R-L}          \\    
\midrule
\textbf{Baselines} \\
BERTSumAbs \cite{liu-lapata-2019-text} &41.7 &19.4 &38.8  \\
$\textrm{T5}_{\textrm{Large}}$ \cite{raffel2020exploring} &42.5 &20.7 &39.8  \\
$\textrm{BART}_{\textrm{Large}}$ \cite{lewis2019bart} &44.2 &21.3 &40.9  \\
PEGASUS \cite{zhang2020pegasus} &44.2 &21.6 &41.3  \\ 
MatchSum \cite{zhong-etal-2020-extractive} &44.4 &20.9 &40.6 \\
GSum \cite{sun2021alleviating} &45.9 &\textbf{22.3} &\textbf{42.5}\\
$\textrm{BigBird}_{\textrm{Large}}$ \cite{zaheer2021big} &43.8 &21.1 &40.7\\
SimCLS \cite{liu-liu-2021-simcls} &\textbf{46.7} &22.2 &\textbf{43.5} \\
SeqCo \cite{xu2022sequence} &45.0 &21.8 &41.8\\
$\textrm{GLM}_{\textrm{RoBERTa}}$ \cite{du-etal-2022-glm} &43.8 &21.0 &40.5 \\
Fourier-BART \cite{he2023fourier} &44.8 &21.6 &41.3 \\
\midrule
\textbf{LLM (zero-shot)} &&& \\
GPT-3.5 (w/o rationale) &37.4 &13.8 &24.1\\
% GPT-3.5 (w/ rationale) &41.6 &18.1 &33.2\\
\midrule
\textbf{Our Method} &&& \\
$\texttt{TriSum-M}$  &\textbf{45.9} &\textbf{22.8} &\textbf{42.3} \\
$\texttt{TriSum-C}$  &45.5 &\textbf{22.3} &41.2 \\
$\texttt{TriSum-J}$  &\textbf{45.6} &\textbf{22.6} &41.9 \\
\midrule
\midrule
  \multicolumn{4}{c}{\textbf{XSum}}    \\      
\textbf{Model} & \textbf{R-1}   & \textbf{R-2}   & \textbf{R-L}          \\
\midrule
\textbf{Baselines} \\
BERTSumAbs \cite{liu-lapata-2019-text} &38.8 &16.3 &31.2  \\
$\textrm{T5}_{\textrm{Large}}$ \cite{raffel2020exploring} &40.9 &17.3 &33.0  \\
$\textrm{BART}_{\textrm{Large}}$ \cite{lewis2019bart} &45.2 &22.3 &37.2  \\
PEGASUS \cite{zhang2020pegasus} &\textbf{47.6} &\textbf{24.8} &\textbf{39.6}  \\ 
MatchSum \cite{zhong-etal-2020-extractive} &24.9 & 4.7 &18.4 \\
GSum \cite{sun2021alleviating} &45.4 &21.9 &36.7\\
$\textrm{BigBird}_{\textrm{Large}}$ \cite{zaheer2021big} &47.1 &24.1 &38.8 \\
SimCLS \cite{liu-liu-2021-simcls} &\textbf{47.6} &24.6 &\textbf{39.4} \\
SeqCo \cite{xu2022sequence} &45.6 &22.4 &37.0\\
$\textrm{GLM}_{\textrm{RoBERTa}}$ \cite{du-etal-2022-glm} &45.5 &23.5 &37.3\\
\midrule
\textbf{LLM (zero-shot)} &&& \\
GPT-3.5 (w/o rationale) \\
\midrule
\textbf{Our Method} &&& \\
$\texttt{TriSum-M}$  &\textbf{48.1} &\textbf{25.2} &\textbf{39.7} \\
$\texttt{TriSum-C}$  &47.5 &24.6 &39.3 \\
$\texttt{TriSum-J}$  &\textbf{47.8} &\textbf{25.0} &\textbf{39.6} \\
\bottomrule
\end{tabular}
}
\caption{\textbf{ROUGE scores on CNN/Daily Mail and XSum datasets with human-annotated summaries}. \texttt{TriSum-M}, \texttt{TriSum-C}, and \texttt{TriSum-J} denote the model checkpoints at the completion of modular learning, concurrent learning, and joint learning, respectively. For \texttt{TriSum-M}, we use the separate optimal checkpoints for different tasks. We highlight top-3 results \textbf{in bold}.}

\label{tb:perf_rouge_scores}
\end{table}

==> tables/perf_plm_scores_general.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!h]
\small
\centering
% \setlength{\tabcolsep}{3.9pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccc}
\toprule
&  \multicolumn{2}{c}{\textbf{CNN/DailyMail}}  & \multicolumn{2}{c}{\textbf{XSum}}  & \multicolumn{2}{c}{\textbf{ClinicalTrial}}  \\      
\textbf{Model} & \textbf{BS}   & \textbf{BAS}   & \textbf{BS}   & \textbf{BAS} & \textbf{BS}   & \textbf{BAS}        \\    
\midrule
$\textrm{T5}_{\textrm{Large}}$ &87.22 &-3.71 &90.73 &-2.70   &90.49 &-1.91 \\
$\textrm{BART}_{\textrm{Large}}$ &87.98 &-3.45 &91.62 &-2.50 &89.61 &-1.99  \\
PEGASUS &87.37 &-3.64 &91.90 &-2.44  &90.16 &-1.61 \\ 
$\textrm{GPT-3.5}_{\textrm{zero-shot}}$  &87.70 &-3.36 &87.67 &-2.80 &89.00 &-2.44\\
\midrule
\textbf{Our Method} &&& \\
$\textrm{GPT-3.5}_{\textrm{rationale}}$ &&&&&&\\
$\texttt{TriSum-S}$ \\
$\texttt{TriSum-C}$ \\
$\texttt{TriSum-R}$ \\

\bottomrule
\end{tabular}
}
\caption{\textbf{Language model-assessed semantic similarity scores on CNNDM, XSum, and ClinicalTrial datasets}. \textbf{BS} and \textbf{BAS} denote BERTScore and BARTScore, respectively.}

\label{tb:perf_plm_scores}
\end{table}

==> tables/perf_rouge_cnn.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!tp]
\small
\centering
% \setlength{\tabcolsep}{3.9pt}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
  \multicolumn{4}{c}{\textbf{CNN/DailyMail}}    \\      
\textbf{Model} & \textbf{R-1}   & \textbf{R-2}   & \textbf{R-L}          \\    
\midrule
\textbf{Baselines} \\
BERTSumAbs \cite{liu-lapata-2019-text} &41.7 &19.4 &38.8  \\
${\textrm{T5}_{\textrm{Large}}}^{*}$ \cite{raffel2020exploring} &42.4 &20.8 &39.9  \\
\greybox{${\textrm{BART}_{\textrm{Large}}}^{*}$} \cite{lewis2019bart} &\greybox{44.0} &\greybox{21.1} &\greybox{40.6}  \\
$\textrm{PEGASUS}^{*}$ \cite{zhang2020pegasus} &44.2 &21.6 &41.3  \\ 
MatchSum \cite{zhong-etal-2020-extractive} &44.4 &20.9 &40.6 \\
GSum \cite{sun2021alleviating} &45.9 &\textbf{22.3} &\textbf{42.5}\\
$\textrm{BigBird}_{\textrm{Large}}$ \cite{zaheer2021big} &43.8 &21.1 &40.7\\
SimCLS \cite{liu-liu-2021-simcls} &\textbf{46.7} &22.2 &\textbf{43.5} \\
SeqCo \cite{xu2022sequence} &45.0 &21.8 &41.8\\
$\textrm{GLM}_{\textrm{RoBERTa}}$ \cite{du-etal-2022-glm} &43.8 &21.0 &40.5 \\
Fourier-BART \cite{he2023fourier} &44.8 &21.6 &41.3 \\
$\textrm{GPT-3.5}_{\textrm{zero-shot}}^{*}$ &37.4 &13.8 &29.1 \\
\midrule
\textbf{Our Method} &&& \\
GPT-3.5 w/ \texttt{TriSum} rationale &46.7 &23.5 &40.7\\
$\texttt{TriSum-S}$  &\textbf{45.9} &\textbf{22.8} &\textbf{42.3} \\
$\texttt{TriSum-C}$  &45.5 &\textbf{22.3} &41.2 \\
$\texttt{TriSum-R}$  &\textbf{45.6} &\textbf{22.6} &41.9 \\
\bottomrule

\end{tabular}
}
\caption{\textbf{ROUGE scores on CNN/Daily Mail dataset}. \texttt{TriSum-S}, \texttt{TriSum-C}, and \texttt{TriSum-R} denote the model checkpoints at the completion of singular-task learning, concurrent learning, and rationale learning, respectively. For \texttt{TriSum-S}, we use the separate optimal checkpoints for different tasks. Models with ``$*$'' are re-evaluated. We highlight top-3 results \textbf{in bold}.}

\label{tb:perf_rouge_cnn}
\end{table}

==> tables/perf_rouge_xsum_clinical.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!tp]
\small
\centering
% \setlength{\tabcolsep}{3.9pt}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
\multicolumn{4}{c}{\textbf{XSum}}    \\      
\textbf{Model} & \textbf{R-1}   & \textbf{R-2}   & \textbf{R-L}          \\
\midrule
\textbf{Baselines} \\
BERTSumAbs \cite{liu-lapata-2019-text} &38.8 &16.3 &31.2  \\
${\textrm{T5}_{\textrm{Large}}}^{*}$ \cite{raffel2020exploring} &40.1 &17.2 &32.3  \\
${\textrm{BART}_{\textrm{Large}}}^{*}$ \cite{lewis2019bart} &45.4 &22.3 &37.3  \\
$\textrm{PEGASUS}^{*}$ \cite{zhang2020pegasus} &\textbf{46.7} &\textbf{24.4} &\textbf{38.9}  \\ 
MatchSum \cite{zhong-etal-2020-extractive} &24.9 & 4.7 &18.4 \\
GSum \cite{sun2021alleviating} &45.4 &21.9 &36.7\\
$\textrm{BigBird}_{\textrm{Large}}$ \cite{zaheer2021big} &47.1 &24.1 &38.8 \\
SimCLS \cite{liu-liu-2021-simcls} &\textbf{47.6} &24.6 &\textbf{39.4} \\
SeqCo \cite{xu2022sequence} &45.6 &22.4 &37.0\\
$\textrm{GLM}_{\textrm{RoBERTa}}$ \cite{du-etal-2022-glm} &45.5 &23.5 &37.3\\
$\textrm{GPT-3.5}_{\textrm{zero-shot}}^{*}$ &26.6 &6.67 &18.80\\
% w/ quality rationale &39.7 &19.2 &32.7\\
\midrule
\textbf{Our Method} &&& \\
GPT-3.5 w/ \texttt{TriSum} rationale &34.4 &12.6 &28.4\\
$\texttt{TriSum-S}$  &\textbf{47.4} &\textbf{24.8} &\textbf{39.4} \\
$\texttt{TriSum-C}$  &46.5 &24.0 &38.7 \\
$\texttt{TriSum-R}$  &\textbf{47.2} &\textbf{24.6} &\textbf{39.0} \\
\midrule
\midrule
\multicolumn{4}{c}{\textbf{ClinicalTrial}}    \\      
\textbf{Model} & \textbf{R-1}   & \textbf{R-2}   & \textbf{R-L}          \\
\midrule
${\textrm{T5}_{\textrm{Large}}}^{*}$ \cite{raffel2020exploring} &53.9 &41.7 &47.2  \\
${\textrm{BART}_{\textrm{Large}}}^{*}$ \cite{lewis2019bart} &51.8 &38.6 &43.6  \\
$\textrm{PEGASUS}^{*}$ \cite{zhang2020pegasus} &51.8 &40.7 &44.8  \\ 
$\textrm{GPT-3.5}_{\textrm{zero-shot}}^{*}$ &45.4 &23.8 &32.5 \\
\midrule
\textbf{Our Method}  \\
GPT-3.5 w/ \texttt{TriSum} rationale &54.1 &37.6 &42.2 \\
$\texttt{TriSum-S}$  &53.6 &42.2 &46.6 \\
$\texttt{TriSum-C}$  &50.3 &37.2 &42.8 \\
$\texttt{TriSum-R}$  &52.9 &41.8 &45.2 \\
\bottomrule

\end{tabular}}
\caption{\textbf{ROUGE scores on XSum and ClinicalTrial dataset}. \texttt{TriSum-S}, \texttt{TriSum-C}, and \texttt{TriSum-R} denote the model checkpoints at the completion of singular-task learning, concurrent learning, and rationale learning, respectively. For \texttt{TriSum-S}, we use the separate optimal checkpoints for different tasks. Models with $*$ are re-evaluated by us. We highlight top-3 results \textbf{in bold}.}

\label{tb:perf_rouge_xsum_clinical}
\end{table}
